Counting list homomorphisms from graphs of bounded treewidth: tight complexity bounds

The goal of this work is to give precise bounds on the counting complexity of a family of generalized coloring problems (list homomorphisms) on bounded-treewidth graphs. Given graphs $G$, $H$, and lists $L(v)\subseteq V(H)$ for every $v\in V(G)$, a {\em list homomorphism} is a function $f:V(G)\to V(H)$ that preserves the edges (i.e., $uv\in E(G)$ implies $f(u)f(v)\in E(H)$) and respects the lists (i.e., $f(v)\in L(v))$. Standard techniques show that if $G$ is given with a tree decomposition of width $t$, then the number of list homomorphisms can be counted in time $|V(H)|^t\cdot n^{\mathcal{O}(1)}$. Our main result is determining, for every fixed graph $H$, how much the base $|V(H)|$ in the running time can be improved. For a connected graph $H$ we define $\operatorname{irr}(H)$ the following way: if $H$ has a loop or is nonbipartite, then $\operatorname{irr}(H)$ is the maximum size of a set $S\subseteq V(H)$ where any two vertices have different neighborhoods; if $H$ is bipartite, then $\operatorname{irr}(H)$ is the maximum size of such a set that is fully in one of the bipartition classes. For disconnected $H$, we define $\operatorname{irr}(H)$ as the maximum of $\operatorname{irr}(C)$ over every connected component $C$ of $H$. We show that, for every fixed graph $H$, the number of list homomorphisms from $(G,L)$ to $H$ * can be counted in time $\operatorname{irr}(H)^t\cdot n^{\mathcal{O}(1)}$ if a tree decomposition of $G$ having width at most $t$ is given in the input, and * cannot be counted in time $(\operatorname{irr}(H)-\epsilon)^t\cdot n^{\mathcal{O}(1)}$ for any $\epsilon>0$, even if a tree decomposition of $G$ having width at most $t$ is given in the input, unless the #SETH fails. Thereby we give a precise and complete complexity classification featuring matching upper and lower bounds for all target graphs with or without loops.

==> coloring.tex <==
In this section we prove the following theorem, whose decision version (conditioned on the SETH) was shown by Lokshtanov, Marx, Saurabh~\cite{DBLP:journals/talg/LokshtanovMS18}.

\begin{thm}\label{thm:coloring}
For every $q \geq 3$, there is no algorithm that, given any $n$-vertex graph and its path decomposition with width at most $t$,
counts all proper $q$-colorings in time $(q-\epsilon)^t \cdot  \poly(n)$ for any $\epsilon >0$, unless the \#SETH fails.
\end{thm}

In general our proof goes along the lines of the proof of the decision version.
However, to increase the clarity of presentation, let us first show an intermediate result, whose decision version was shown by Lampis~\cite{DBLP:journals/siamdm/Lampis20}. Our proof is just an adaptation of the original one to the counting world, so we will not elaborate on the details and refer the reader to the paper of Lampis~\cite{DBLP:journals/siamdm/Lampis20}.
For integers $r,q \geq 2$, by \CSP($q$,$r$) we denote the CSP problem with domain $[q]$ and each constraint of arity at most $r$.
By \#\CSP($q$,$r$) we denote the problem of counting satisfying valuations of a given instance of \CSP($q$, $r$).


\begin{thm}\label{thm:qcsp}
For every integer $q \geq 2$ and $\epsilon >0$ there is an integer $r$, such that the following holds.
Unless the \#SETH fails, \#\CSP($q$,$r$) with $n$ variables and $m$ constraints cannot be solved in time $(q-\epsilon)^n \cdot \poly(n + m)$.
\end{thm}

\begin{proof}
Fix $q \geq 2$ and $\epsilon > 0$ and suppose that for every $r$ there is an algorithm solving $n$-variable $m$-constraint \#\CSP($q$, $r$) in time $(q-\epsilon)^n \cdot \poly(n + m)$.
Suppose we are given a $s$-\textsc{SAT} instance $\Phi$ with $N$ variables and $M$ clauses, where $s$ is a constant.
Without loss of generality we may assume that each variable is involved in some clause.

In the reduction we will carefully choose $r = r(s,q,\epsilon)$ and build a \CSP($q$, $r$) instance $\Psi$.
To avoid confusion, we will refer to an assignment of values to the variables of $\Phi$ as \emph{truth assignment},
while an assignment of values to the variables of $\Psi$ will be called \emph{valuation}.

First, select an integer $p$ and a real $\delta > 0$, such that there exists an integer $t$ satisfying the following (see~\cite{DBLP:journals/siamdm/Lampis20} for the argument that such a choice is possible):
\[
(q-\epsilon)^p \leq (2-\delta)^t \leq 2^t \leq q^p.
\]
Now group the variables of $\Phi$ into $\gamma := \lceil N/t \rceil$ groups, each with at most $t$ variables.
Call these groups $V_1,V_2\ldots,V_\gamma$.
For each $i \in [\gamma]$, we create a group $X_i$ of $p$ variables of $\Psi$.
Thus the total number of variables in $\Psi$ is $n:= \gamma \cdot p \leq \frac{pN}{t} + p$.

Note that the total number of truth assignments of variables in $V_i$ is at most $2^t \leq q^p$, so it does not exceed the number of possible valuations of $X_i$. Let us fix some injective function that maps each truth assignment on $V_i$ to a distinct valuation of $X_i$.

Now, let us define the constraints of $\Psi$.
Consider any clause $c$ of $\Phi$ and let $V_{i_1},V_{i_2},\ldots,V_{i_{s'}}$ for $s' \leq s$ be the groups that contain the variables of $c$.
Note that each truth assignment of variables in $V_{i_1},V_{i_2},\ldots,V_{i_{s'}}$ that satisfies $c$ corresponds to some valuation of variables in $X_{i_1},X_{i_2},\ldots,X_{i_{s'}}$.
We introduce a new constraint $C(c)$ on all variables from $X_{i_1} \cup X_{i_2} \cup \ldots \cup X_{i_{s'}}$ that accepts only the valuations that correspond to the truth assignments that satisfy $c$.
The arity of $C(c)$ is  $|X_{i_1} \cup X_{i_2} \cup \ldots \cup X_{i_{s'}}| \leq s \cdot p$.

Summing up, $\Psi$ has  $n= \gamma \cdot p \leq \frac{pN}{t} + p$ variables, $m = M$ constraints, its domain is $[q]$, and each constraint has arity at most $r := sp$.

It is straightforward to observe that $\Phi$ has a satisfying truth assignment if and only if $\Psi$ has a satisfying valuation.
However, a stronger property holds as well: there is a bijection between truth assignments that satisfy $\Phi$ and valuations that satisfy $\Psi$.
Indeed, recall that every variable of $\Phi$ appears in some clause, and thus, for each $i\in[\gamma]$, there is a constraint of $\Psi$ involving all variables of $X_i$. Since the constrains of $\Psi$ were defined in a way that the only accepted valuations are in one-to-one correspondence to the truth assignments of $\Phi$, we observe that the claimed bijection between truth assignments and valuations exists.
Hence, the solution to \CSP($q$, $r$) on the instance $\Psi$ is precisely the number of satisfying assignments of $\Phi$.
Let us call our hypothetical algorithm for $\Psi$. Its running time is:
\begin{align*}
(q - \epsilon)^n \cdot \poly(n + m) \leq & \left((q - \epsilon)^p\right)^{N/t+1} \cdot \poly(N + M)
 \leq \left((2 - \delta)^t\right)^{N/t+1} \cdot \poly(N+M) \\ \leq & 2^t \cdot (2-\delta)^{N} \cdot \poly(N+M).
\end{align*}
As $t$ depends only on $q$ and $\epsilon$, this running time is $(2-\delta)^{N} \cdot \poly(N+M)$, which violates the \#SETH.
\end{proof}

Now we are ready to prove Theorem~\ref{thm:coloring}. Similarly to the proof of Theorem~\ref{thm:qcsp},
it is an adaptation of the proof of Lokshtanov, Marx, Saurabh~\cite{DBLP:journals/talg/LokshtanovMS18} to the counting setting.

\begin{proof}[Proof of Theorem~\ref{thm:coloring}.]
Suppose that there is $\epsilon >0$ and an algorithm that counts proper $q$-colorings
of each graph with $n$ vertices, given with a path decomposition of width at most $t$, in time $(q-\epsilon)^{t} \cdot \poly(n)$.
Consider an instance $\Psi$ of \CSP($q$, $r$) with $N$ variables $\{v_1,v_2,\ldots,v_N\}$ and $M$ constraints.
We will show that our hypothetical algorithm can be solved to count satisfying valuations of $\Psi$
in time $(q-\epsilon)^N \cdot \poly(N + M)$, which, by Theorem~\ref{thm:qcsp}, contradicts the \#SETH.

\paragraph{Constructing an instance of $q$-coloring.}
As the first step, let us build a graph $G$ with list function $L \from V(G) \to 2^{[q]}$,
such that $G$ has a proper coloring respecting the lists $L$ if and only if $\Psi$ is satisfiable.

First, we introduce to $G$ vertices $V := \{v_1,v_2,\ldots,v_N\}$, i.e., the variables of $\Psi$.
Each vertex of $V$ has list $[q]$. Coloring the vertex $v_i$ with one of $q$ possible colors will in
a natural way correspond to assigning this value to the variable $v_i$.

Now consider a constraint $C$ of $\Psi$ and let $V(C)$ be the set of variables appearing in $C$.
Let $p$ be the number of valuations of $V(C)$ that satisfy $C$; note that $p \leq q^r$.
We introduce to $G$ a path $P_C$ with $p$ vertices $z_1,z_2,\ldots,z_p$, each with lists $\{1,2,3\}$.
These vertices are in one-to-one correspondence with the valuations of $V(C)$ that satisfy $C$.
Furthermore, we add two new vertices: $z_0$, which is adjacent to $z_1$ only, and $z_{p+1}$, which is adjacent to $z_p$ only.
Note that we do not count these two vertices to be a part of $P_C$.
We set $L(z_0) = \{2\}$. The list of $z_2$ depends on the parity of $p$: we set $L(z_{p+1}) = \{2\}$ if $p$ is even,
and $L(z_{p+1}) = \{3\}$ if $p$ is odd.
Observe that in order to find a list coloring of vertices of $P_C$, there must be some $i \in [p]$,
such that the vertex of $z_i$ receives the color 1. This will correspond to choosing the valuation of $V(C)$ that corresponds to $z_i$.
Let $Z$ be the set of vertices constructed in this step, i.e., the vertices of paths $P_C$ and the additional pending vertices,
two for each path.

The only thing left is to ensure that a vertex $z$ from a path $P_C$ can be colored 1 if and only if
the coloring of vertices from $V(C)$ is precisely the valuation corresponding to $z$.
Fix some $z$ from a path $P_C$ and let $f \from V(C) \to [q]$ be the valuation corresponding to $z$.
Let $v \in V(C)$ and let $i := f(v)$.
We will build a constant-size gadget $F_i$ with lists $L$, called a \emph{connector}, intersecting $V \cup Z$ only in $\{v,z\}$, such that
\begin{align*}
& \{ (h(v),h(z)) ~|~ h \text{ is a a proper coloring of $F_i$ respecting lists $L$} \}  \\ &=  \{ (i,1) \} \cup \{ (i,2),(i,3) ~|~ i \in [q] \setminus \{i\} \}.  
\end{align*}
The ordered pair $(v,z)$ is called the \emph{interface} of the connector. The other vertices are called \emph{internal}.
One can readily verify that if we are able to build a connector for every relevant pair $v,z$,
then the constructed graph admits a proper list $q$-coloring if and only if $\Psi$ is satisfiable,
see also~\cite{DBLP:journals/talg/LokshtanovMS18}.

So let us fix a pair of vertices $v,z$ and the color $i=f(v)$ as above, and let us show how to construct a connector.
We note that such a gadget can be obtained by constructing, for every $j \in [q] \setminus \{i\}$,
a constant-size gadget $\overline{F}_j$ with lists $L$, intersecting $V \cup Z$ only in $\{v,z\}$, such that
\begin{align*}
\{ (h(v),h(z)) ~|~ h \text{ is a a proper coloring of $\overline{F}_j$ respecting lists $L$} \}  =  [q] \times [3] \setminus \{(j,1)\}.  
\end{align*}
The construction of such gadgets is depicted in Figure~\ref{fig:coloring-gadgets}, see~\cite{DBLP:journals/talg/LokshtanovMS18} for the details.
Observe that each gadget $\overline{F}_j$ has at most 7 vertices, except for $\{v,z\}$.
Thus each connector has at most internal $7q$ vertices. Let $M'$ be the total number of connectors, note that $M' \leq M \cdot q^r$.
\begin{figure}
\centering
\includegraphics[scale=1]{figs-coloring}
\caption{The construction of the gadget $\overline{F}_j$ for $j=1$ (left) and for $j \neq 1$ (right). The sets indicate the lists $L$.
Moreover, $L(v) = [q]$ and $L(z) = [3]$.}
\label{fig:coloring-gadgets}
\end{figure}

This completes the construction of $(G,L)$. Now let us turn it into an equivalent instance $G_1$ of (non-list) $q$ coloring.
We introduce $q$ new vertices $W=\{w_1,\ldots,w_q\}$ and make them pairwise adjacent. As in every proper $q$-coloring, each vertex of $W$ must receive a distinct color, we will use the coloring of these vertices as a reference coloring.
Now for every vertex $u$ of $G$, and every $i \notin L(u)$ we add an edge joining $u$ and $w_i$.
It is straightforward to verify that $G$ has a proper $q$-coloring respecting the lists $L$ if and only if $G_1$ has a proper $q$-coloring.

\paragraph{Constructing the family of graphs $G_d$.}
Now, for an integer $d \geq 2$, let $G_d$ be the graph obtained from $G_1$ by replacing each connector with its $d$ copies, sharing their corresponding interface vertices $v$ and $z$ (i.e., only internal vertices of connectors are duplicated).
Let us summarize some properties of each instance $G_d$ constructed this way.
First, $G_d$ has a proper $q$-coloring if and only if $\Psi$ has a satisfying valuation.
Next, the number of vertices of $G_d$ is at most 
\begin{equation}
\underbrace{N}_{V}+ \underbrace{M \cdot (q^r+2)}_{Z}+ \underbrace{d \cdot M' \cdot 7q}_{\text{connectors}} + \underbrace{q}_{W} = N + \bigO(M) + \bigO(dM) = \bigO(N+ dM). \label{eq:Gd-vertices}
\end{equation}

Finally, let us construct a path decomposition of $G_d$ with width at most $N+8q+1$.\prz{this can be improved to $\approx N+7 + q+1$ by noting that connectors consists of independent pieces, and to $\approx N+q+3$ by additionally analyzing these pieces, but I don't think we care.}
Let us fix an arbitrary ordering of constraints of $\Psi$ and create a path decomposition $\calX = (X_1,\ldots,X_s)$ of $G_d[Z]$ by concatenating optimal path decompositions of consecutive paths $P_C$.
Clearly, the size of each set $X_i$ is at most 2.
Next, take a vertex $z$ in some path $P_C$ and let $X_i$ be the first bag of $\calX$ containing $z$.
Recall that $z$ is contained in $d$ connectors.
Between $X_i$ and $X_{i+1}$ we insert $d$ copies of $X_i$, and to each of these copies we add all internal vertices of a distinct connector containing $z$.
Let $\calX'$ be a sequence obtained from $\calX$ by repeating this step for every vertex $z$ of every path $P_C$.
Note that $\calX'$ is a path decomposition of $D_d - (V \cup W)$, and its width is at most $1 + 7q$.
Finally, we turn $\calX'$ into a path decomposition of $G_d$ with width at most $1 + 8q + N$ by adding $V \cup W$ to every bag.

Let $\boldb_d$ be the number of proper $q$-colorings of $G_d$.
Recall that by our assumption we can compute $\boldb_d$ in time
\begin{equation}
(q-\epsilon)^{N+8q+1} \cdot \poly(N+dM) = (q-\epsilon)^N \cdot \poly(N + dM).
\label{eq:one-call}
\end{equation}
Thus, in order to reach a contradiction, it is sufficient to show that knowing $\boldb_d$ for all $d \in [D]$, where $D$ is some value polynomial in $M$, we can compute the number of satisfying valuations of $\Psi$. We will argue that this is possible using Lemma~\ref{lem:interpolation}.

\paragraph{Colorings of $G_d$ and valuations of $\Psi$.}
For each permutation $\pi \from [q] \to [q]$, let $\boldb_d^\pi$ be the number of proper $q$-colorings $f$ of $G_d$,
such that $f(w_i) = \pi(i)$ for every $i \in [q]$. Clearly $\boldb_d  = \sum_{\pi} \boldb_d^\pi$.
By the symmetry of the problem we observe that $\boldb_d^\pi = \boldb_d^{\pi'}$ for all $\pi,\pi'$.
Thus, setting $\boldb_d' := \boldb_d^{\mathrm{identity}}$, we conclude that $\boldb_d = q! \cdot \boldb_d'$.
So from now on let us focus on proper $q$-colorings of $G_d$ that color each $w_i$ with color $i$; we call them \emph{canonical}.
Note that canonical colorings respects lists $L$.

For a canonical coloring $f$, its \emph{template} is the restriction of $f$ to $V$.
For each $q$-coloring $h$ of $V$, let $\mathsf{ext}_d(h)$ be the set of canonical colorings of $G_d$ whose template is $h$.
Note that the construction of $G_d$ ensures that for all $d,d'$, either both sets $\mathsf{ext}_d(h),\mathsf{ext}_{d'}(h)$ are empty, or both are nonempty  -- this comes from the fact that all copies of the same connector gadget can receive the same coloring.
Let $\mathsf{Val}$ be the set $q$-colorings $h$ of $V$, such that $\mathsf{ext}_1(h) \neq \emptyset$.
Clearly we have
\begin{equation}
\boldb_d' = \sum_{h \from V \to [q]} |\mathsf{ext}_d(h)| = \sum_{h \in \mathsf{Val}} |\mathsf{ext}_d(h)|.
\label{eq:bdprime}
\end{equation}

Let us now discuss some properties of elements of $\mathsf{Val}$.
First, note that $h \in \mathsf{Val}$ if and only if $h$ corresponds to a satisfying valuation  of $\Psi$.
Thus counting the number of satisfying valuations of $\Psi$ boils down to computing $|\mathsf{Val}|$.

Second, we observe that if $f,f' \in \mathsf{ext}_d(h)$, then $f|_Z = f'|_Z$. This comes the fact that having fixed the coloring of $V$ corresponding to a satisfiable valuation of $\Psi$, there is exactly one vertex on each path $P_C$ that receives color 1.
In other words, the way some canonical coloring colors the set $Z$ is uniquely determined by its template.
So from now on, if it does not lead to confusion, we will treat each $h \in \mathsf{Val}$ as a $q$-coloring of $V \cup Z$.

Note that the discrepancy in the values of $|\mathsf{ext}_d(h)|$ for distinct $d$ comes from the fact that colorings of internal vertices of connector gadgets are not unique.
So now let us analyze how connector gadgets can be colored.
Recall that we have $q$ distinct types of connector gadgets: $F_1,F_2,\ldots,F_q$.\prz{again, this is in fact smaller since there are essentially two types of connectors, but I don't think we care}
Recall that we only consider canonical colorings, so we may imagine that each vertex of each connector gadget has a list of allowed colors.

For $i \in [q]$ and consider a connector gadget $F_i$ with interface $(v,z)$.
For $j \in [q]$, $\ell \in [3]$, let $c(i,j,\ell)$ be the number of proper $q$-colorings of $F_i$ (respecting lists),
such that the color of $v$ is $j$ and the color of $z$ is $\ell$.
Recall from the construction of connector gadgets that if $\iota \in [q] \times [q] \times [3]$, then $c(\iota) \neq 0$
if and only if $\iota \in \mathcal{I} := \{ (i,j,\ell) \in [q] \times [q] \times [3] ~|~ i=j \lor \ell \neq 1 \}$.

Let $\mathsf{sgn} \from \mathsf{Val} \times \mathcal{I} \to \N$ be the function that, for each $h \in \mathsf{Val}$ and $(i,j,\ell) \in  \mathcal{I}$, counts the number of connector gadgets $F_i$ in $G_1$, such that $h(v)=j$ and $h(z)=\ell$, where $(v,z)$ is the interface of $F_i$. Note that the number of analogous gadgets in $G_d$ is exactly $d \cdot \mathsf{sgn}(h,(i,j,\ell))$.
We obtain
\[
|\mathsf{ext}_1(h)| = \prod_{\iota \in \mathcal{I}} c(\iota)^{\mathsf{sgn}(h,\iota)}\]
and consequently
\begin{equation}
|\mathsf{ext}_d(h)| = \prod_{\iota \in \mathcal{I}} c(\iota)^{d \cdot \mathsf{sgn}(h,\iota)} = \left(\prod_{\iota \in \mathcal{I}}c(\iota)^{\mathsf{sgn}(h,\iota)}\right)^d.
\label{eq:extd}
\end{equation}

For $h \in \mathsf{Val}$, define $\boldw(h) :=  \prod_{\iota \in \mathcal{I}} c(\iota)^{\mathsf{sgn}(h,\iota)}$.
Recall that for each $h \in \mathsf{Val}$ we have $\boldw(h) >0$.
Let $\boldW := \{  \boldw(h) ~|~ h \in \mathsf{Val} \}$, and for $\boldw \in \boldW$,
let $\mathsf{val}(w)$ be the set of $h \in \mathsf{Val}$, such that $\boldw(h) = \boldw$.

Combining \eqref{eq:bdprime} and \eqref{eq:extd}, we obtain
\begin{align*}
\boldb_d / q! = &  \boldb_d' = \sum_{h \in \mathsf{Val}} |\mathsf{ext}_d(h)| =\left(\prod_{\iota \in \mathcal{I}}c(\iota)^{\mathsf{sgn}(h,\iota)}\right)^d \\
= &  \sum_{h \in \mathsf{Val}} \boldw(h)^d = \sum_{\boldw \in \boldW} \boldw^d \cdot |\mathsf{val}(\boldw)|.
\end{align*}

Thus, having computed $\boldb_d$ for all $d \in [|\boldW|]$, we can use Lemma~\ref{lem:interpolation} to determine the value of $|\mathsf{val}(\boldw)|$ for each $\boldw$. As
\[
|\mathsf{Val}| = \sum_{\boldw \in \boldW} |\mathsf{val}(\boldw)|,
\]
this allows us to compute the number of colorings in $\mathsf{Val}$ and thus the number of satisfying valuations of $\Psi$.
The last thing to do it to estimate $|\boldW|$ to argue about the running time of our algorithm.
Recall that the number of connector gadgets in $G_1$ is $M' \leq M \cdot q^r$.
The number of possible values $\boldw \in \boldW$ is upper bounded by the number of partitions of $M'$ to $3q^2$ summands, which is in turn upper-bounded by 
\[
M'^{3q^2} \leq (M \cdot q^r)^{3q^2}.
\]
Summing up, we can compute the number of satisfying valuations of $\Psi$ by calling our hypothetical algorithm for counting proper $q$-colorings for at most $\bigO(M^{3q^2})$ instances. Each instance has pathwidth at most $N+8q+1$ and, by \eqref{eq:Gd-vertices},
\[
\bigO(N + M^{3q^2} \cdot M)
\]
vertices.
By \eqref{eq:one-call}, the complexity of each call is at most
\[
(q-\epsilon)^N \cdot \poly(N + M^{3q^2+1}) = (q-\epsilon)^N \cdot \poly(N + M),
\]
as $q$ is constant. Thus one can solve an $N$-vertex $M$-constraint \#\CSP($q$,$r$) in time $(q-\epsilon)^N \poly(N + M)$, which violates the \#SETH by Theorem~\ref{thm:qcsp}.
\end{proof}
